On Deterministic Conditions for Subspace Clustering under Missing Data

In this paper we present deterministic conditions for success of sparse subspace clustering (SSC) under missing data, when data is assumed to come from a Union of Subspaces (UoS) model. We consider two algorithms, which are variants of SSC with entry-wise zero-filling that differ in terms of the optimization problems used to find affinity matrix for spectral clustering. For both the algorithms, we provide deterministic conditions for any pattern of missing data such that perfect clustering can be achieved. We provide extensive sets of simulation results for clustering as well as completion of data at missing entries, under the UoS model. Our experimental results indicate that in contrast to the full data case, accurate clustering does not imply accurate subspace identification and completion, indicating the natural order of relative hardness of these problems.

==> apdx_full.tex <==
\section{Toconsider:maybe bot neeeded: Proof of Remark  \ref{corollary1}: Theorems \ref{theorem} and \ref{corollary3} reduce to Theorem 7 in \cite{dim_red_sc_ext}}\label{apdx:full}

In the case that data are fully observed with no missing entries, ${\bf I}_{\Omega_i^{(l)}}$ and ${\bf I}_{\Omega_j^{(k)}}$ in Theorem \ref{theorem} becomes identity matrix ${\bf I} \in \mathbb{R}^{n\times n}$. Also, data from the same subspace $\mathbb{S}^{(l)}$ has the same bases ${\bf U}^{(l)}$.

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c}
      \includegraphics[scale=0.3]{FullCase.png}
 \end{tabular}}
  \caption{ Full Observation case. $\bf{U}^{(l)} = \bf{Q}^{(l)} {\bf \Sigma}^{(l)} (\bf{R}^{(l)})^\top$ is the SVD, $\underline{\bf{U}}^{(l)}$ is the null space bases of $\bf{U}^{(l)}$}
  \label{fig:Case1}
\end{figure}

The SVD of subspace bases matrix ${\bf U}^{(l)}$ is shown in Fig \ref{fig:Case1}, where ${\bf Q}^{(l)}$ consists exactly ${\bf U}^{(l)}$ and the  null space bases of ${\bf U}^{(l)}$ ( denoted as $\underline{\bf U}^{(l)}$), ${\bf \Sigma}^{(l)}$ is a projection from $\mathbb{R}^{d}$ to $\mathbb{R}^{n}$ that keeps the first $d$ entires  the same and zero-fills the remaining $n-d$ entires,  and ${\bf R}^{(l)}$ becomes an identity matrix. $\tilde{\bf a}_i^{(l)}$ from \eqref{eq: notation_a} becomes
\begin{equation} \label{eq: c1_1}
\tilde{\bf a}_i^{(l)} = {\bf \Sigma} ^{(l)} ({\bf R}^{(l)})^\top {\bf a}_i^{(l)} = 
\begin{bmatrix}
{\bf a}_i^{(l)}\\
{\bf 0}
\end{bmatrix},
\end{equation}
From \eqref{eq: base_groups} and \eqref{eq: c1_1}, we  have
\begin{equation}\label{eq: c1_2}
\tilde{{\bf A}}_{-i}^{(l)} = {\bf \Sigma} ^{(l)} ({\bf R}^{(l)})^\top {{\bf A}}_{-i}^{(l)} ,
\end{equation}

Based on \eqref{eq: c1_1},  the projection from ${\bf a}_i^{(l)}$ to $\tilde{\bf a}_i^{(l)}$ only adds $n-d$ zeros to ${\bf a}_i^{(l)}$ without changing the relative location of data, thus 
the geometry of the body ${\bf A}_{-i}^{(l)}$ is the same as  $\tilde{{\bf A}}_{-i}^{(l)}$, indicating  
\begin{equation}\label{eq: c1_A}
r(\mc{P}({{\bf A}}_{-i}^{(l)})) = r(\mc{P}(\tilde{{\bf A}}_{-i}^{(l)})),
\end{equation}

Let ${\V \lambda}_i^{(l)} \in \arg \max_{\V \lambda} \langle \tilde{{\bf a}}_i^{(l)}, {\V \lambda} \rangle \quad s.t. \quad \|(\tilde{{\bf A}}_{-i}^{(l)})^\top {\V \lambda}\|_\infty \leq 1$. 
From  \eqref{eq: c1_1} \eqref{eq: c1_2}, we have
\begin{equation}
\begin{split}
& {\V \lambda}_i^{(l)} \in \arg \max_{\V \lambda} \langle {{\bf a}}_i^{(l)}, {\bf R}^{(l)} ({\bf \Sigma}^{(l)})^\top{\V \lambda} \rangle \quad \\
& s.t. \quad \|( {{\bf A}}_{-i}^{(l)})^\top \left( {\bf R}^{(l)} ({\bf \Sigma}^{(l)})^\top \right) {\V \lambda}\|_\infty \leq 1.
\end{split}
\end{equation}

Let 
\begin{equation}
\bar{{\V \lambda}}_i^{(l)} \in \arg \max_{\V \lambda} \langle {{\bf a}}_i^{(l)}, {\V \lambda} \rangle \quad s.t. \quad \|({{\bf A}}_{-i}^{(l)})^\top {\V \lambda}\|_\infty \leq  1,
\end{equation}
which gives
\begin{equation} \label{eq: tp_eq}
\bar{{\V \lambda}}_i^{(l)} =  {\bf R}^{(l)} ({\bf \Sigma}^{(l)})^\top{{\V \lambda}}_i^{(l)}.
\end{equation}

Since $({\bf R}^{(l)})^\top$ is an identity matrix and ${\bf \Sigma}^{(l)}$ is also an identity like matrix as shown in Fig \ref{fig:Case1}
\begin{equation}\label{eq: c1_3}
{{\V \lambda}}_i^{(l)} = {\bf \Sigma}^{(l)} ({\bf R}^{(l)})^\top \bar{{\V \lambda}}_i^{(l)} = \begin{bmatrix} \bar{{\V \lambda}}_i^{(l)} \\ {\bf 0} \end{bmatrix},
\end{equation}
 is one of the solution that satisfies \eqref{eq: tp_eq}. Thus

\begin{equation}\label{eq: c1_4}
\|\bar{{\V \lambda}}_i^{(l)}\|_2 = \|{{\V \lambda}}_i^{(l)}\|_2.
\end{equation}

Plugging \eqref{eq: c1_A} \eqref{eq: c1_3} \eqref{eq: c1_4} into \eqref{eq: theorem_eq} gives
\begin{equation}\label{eq: theorem_full}
\left| 
\frac{({\bf \Sigma}^{(l)}  ({\bf R}^{(l)})^\top \bar{{\V \lambda}}_i^{(l)})^\top} {\|(\bar{{\V \lambda}}_i^{(l)})^\top\|_2} ({\bf Q}_i^{(l)})^\top
{\bf U}^{(k)} {\bf a}_j^{(k)}
\right|
< r(\mc{P}({{\bf A}}_{-i}^{(l)})),
\end{equation}
Since $({\bf U}^{(l)})^\top = ({\bf U}^{(l)})^\dagger = {\bf R}^{(l)} ({\bf \Sigma}^{(l)})^\top ({\bf Q}^{(l)})^\top$, thus \eqref{eq: theorem_full} becomes
\begin{equation}
\left| 
\frac{(\bar{{\V \lambda}}_i^{(l)})^\top} {\|\bar{{\V \lambda}}_i^{(l)}\|_2} 
({\bf U}^{(l)})^\dagger
{\bf U}^{(k)} {\bf a}_j^{(k)}
\right|
< r(\mc{P}({{\bf A}}_{-i}^{(l)})),
\end{equation}
which is consistent with the result in [Theorem 7 in \cite{dim_red_sc_ext}].



==> apdx_unif.tex <==
\section{Proof of Theorem \ref{thm:1}: Same Location Sampling Case}\label{apdx:same}
%\begin{proof}
In the case when all the data points are sampled at the same locations, ${\bf I}_{\Omega_i^{(\ell)}} = {\bf I}_{\Omega_j^{(k)}} = {\bf I}_{\Omega}$. 
The modified bases ${\bf V}_\Omega^{(\ell)}$ of $\mathbb{S}^{(\ell)}$ gives 
\begin{equation}
{\bf V}_{\Omega}^{(\ell)} = {\bf Q}^{(\ell)} {\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top,
\end{equation}
where ${\bf Q}^{(\ell)}, {\bf \Sigma}^{(\ell)}$ and ${\bf R}^{(\ell)}$ are subspace dependent and data independent.
 Equations \eqref{eq: base} , \eqref{eq: base_groups} and \eqref{eq: notation_a} gives 
\begin{equation}\label{eq: c2_1}
\begin{split}
& \tilde{{\bf a}}_j^{(k)} = ({\bf Q}_i^{(\ell)})^\top {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)}, \\
& \tilde{{\bf A}} _{-i}^{(\ell)} =  {\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {{\bf A}} _{-i}^{(\ell)}, \\
& \tilde{\bf{a}}_i^{(\ell)} = {\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {\bf a}_i^{(\ell)}, \\
\end{split}
\end{equation} 

Substituting \eqref{eq: c2_1} into \eqref{eq: remark_eq} gives that the deterministic condition holds if the following condition satisfies, 
\begin{equation} \label{eq: 1}
\left| \frac{( {\V \lambda}_i^{(\ell)} )^\top }{\|{\V \lambda}_i^{(\ell)}\|_2} ({\bf Q}^{(\ell)})^\top {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)} \right| 
< r(\mc{P}({\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {{\bf A}} _{-i}^{(\ell)})),
\end{equation}
where 
\begin{equation} \label{eq: 2}
\begin{split}
& {\V \lambda}_i^{(\ell)} \in \arg \max_{\V \lambda} \langle {\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {\bf a}_i^{(\ell)}, {\V \lambda} \rangle \quad \\
& s.t. \quad \|( {\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {{\bf A}} _{-i}^{(\ell)})^\top {\V \lambda}\|_\infty \leq 1.
\end{split}
\end{equation}

Since ${\bf Q}^{(\ell)}$ is a unitary matrix, \eqref{eq: 1} is equivalent to 
\begin{equation} \label{eq: 2.5}
\left| \frac{ ({\bf Q}^{(\ell)} \V {\lambda}_i^{(\ell)} )^\top }{\|{\bf Q}^{(\ell)} \V{\lambda}_i^{(\ell)}\|_2}  {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)} \right| 
< r(\mc{P}({\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {{\bf A}} _{-i}^{(\ell)})).
\end{equation}

In addition, unitary matrix can be regarded as rotation transformation which does not change the shape, thus RHS of \eqref{eq: 2.5} is
\begin{equation}
\begin{split}
& r(\mc{P}({\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {{\bf A}} _{-i}^{(\ell)})) \\
& = r(\mc{P}({\bf Q}^{(\ell)} {\bf \Sigma}^{(\ell)} ({\bf R}^{(\ell)})^\top {{\bf A}} _{-i}^{(\ell)})) \\
& =r(\mc{P}({\bf V}_\Omega^{(\ell)} {{\bf A}} _{-i}^{(\ell)})).
\end{split}
\end{equation}

Equation \eqref{eq: 1} then becomes 
\begin{equation} \label{eq: 3}
\left| \frac{ ({\bf Q}^{(\ell)} \V {\lambda}_i^{(\ell)} )^\top }{\|{\bf Q}^{(\ell)} \V{\lambda}_i^{(\ell)}\|_2}  {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)} \right| 
<r(\mc{P}({\bf V}_\Omega^{(\ell)} {{\bf A}} _{-i}^{(\ell)})).
\end{equation}

Without changing the problem, we insert an identity matrix $({\bf Q}^{(\ell)})^\top {\bf Q}^{(\ell)} = {\bf I} \in \mathbb{R}^{n\times n}$ in front of $\V{\lambda}$ in \eqref{eq: 2} and get
\begin{equation} \label{eq: 4}
\begin{split}
& \V{\lambda}_i^{(\ell)} \in \arg \max_\V{ \lambda} \langle  {\bf a}_i^{(\ell)}, ({\bf V}_\Omega^{(\ell)})^\top {\bf Q}^{(\ell)}\V{ \lambda} \rangle \quad \\
& s.t. \quad \|( {{\bf A}} _{-i}^{(\ell)})^\top ({\bf V}_\Omega^{(\ell)})^\top  {\bf Q}^{(\ell)} {\V \lambda}\|_\infty \leq 1.
\end{split}
\end{equation}

Let $\tilde{\V{\lambda}}_i^{(\ell)} = {\bf Q}^{(\ell)} \V{\lambda}_i^{(\ell)}$, then \eqref{eq: 3} becomes
\begin{equation} \label{eq: 5}
\left| \frac{ ( \tilde{ \V {\lambda}}_i^{(\ell)} )^\top }{\| \tilde{ \V{\lambda}}_i^{(\ell)}\|_2}  {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)} \right| 
< r(\mc{P}({\bf V}_\Omega^{(\ell)} {{\bf A}} _{-i}^{(\ell)})),
\end{equation}
and \eqref{eq: 4} becomes
\begin{equation} \label{eq: 6}
\begin{split}
& \tilde{\V{\lambda}}_i^{(\ell)} \in \arg \max_\V{ \lambda} \langle  {\bf a}_i^{(\ell)}, ({\bf V}_\Omega^{(\ell)})^\top \V{ \lambda} \rangle \quad \\
& s.t. \quad \|( {{\bf A}} _{-i}^{(\ell)})^\top ({\bf V}_\Omega^{(\ell)})^\top  {\V \lambda}\|_\infty \leq 1.
\end{split}
\end{equation}

Further set $\bar{\V{\lambda}}_i^{(\ell)}$ to be the solution to the following optimization problem,
\begin{equation} \label{eq: 7}
\begin{split}
&  \max_\V{ \lambda} \langle  {\bf a}_i^{(\ell)},\V{ \lambda} \rangle \quad \\
& s.t. \quad \|( {{\bf A}} _{-i}^{(\ell)})^\top  {\V \lambda}\|_\infty \leq 1.
\end{split}
\end{equation}

As $\tilde{\V{\lambda}}_i^{(\ell)} = (({\bf V}_\Omega^{(\ell)})^\top)^\dagger \bar{\V{\lambda}}_i^{(\ell)}$ is one of the optimal solutions which satisfies \eqref{eq: 6},
thus plugging $\tilde{\V{\lambda}}_i^{(\ell)}$ into \eqref{eq: 5} indicates
\begin{equation} \label{eq: 8}
\left| { ( \bar{ \V {\lambda}}_i^{(\ell)} )^\top }   ({\bf V}_\Omega^{(\ell)})^\dagger  {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)} \right| 
< r(\mc{P} ({\bf V}_\Omega^{(\ell)} {{\bf A}} _{-i}^{(\ell)}))\times {\| \tilde{ \V{\lambda}}_i^{(\ell)}\|_2}.
\end{equation}

The constraint in \eqref{eq: 6} gives 
\begin{equation}\label{eq: 57}
\|\tilde{\V{\lambda}}_i^{(\ell)} \|_2 \leq R(\mc{P}^o ({\bf V}_\Omega^{(\ell)} {\bf A}_{-i}^{(\ell)})),
\end{equation}
and
\begin{equation}\label{eq: 61}
\| ({\bf V}_\Omega^{(\ell)})^\top  \tilde{\V{\lambda}}_i^{(\ell)} \|_2 \leq R(\mc{P}^o ({\bf A}_{-i}^{(\ell)}) ).
\end{equation}

Based on \eqref{eq: 57} and \eqref{eq: 61}, without loss of generality, let 
\begin{equation}
\|\tilde{\V{\lambda}}_i^{(\ell)} \|_2 = \beta_1 R(\mc{P}^o ({\bf V}_\Omega^{(\ell)} {\bf A}_{-i}^{(\ell)})) , \beta_1 \in [0,1].
\end{equation} 
%From Lemma \ref{lemma1}, we get
%\begin{equation}\label{eq: equal1}
%\|\tilde{\V{\lambda}}_i^{(\ell)} \|_2 =\frac{\beta}{r(\mc{P}( {\bf V}_{\Omega}^{(\ell)} {{\bf A}} _{-i}^{(\ell)})}.
%\end{equation}
and
\begin{equation}
\| ({\bf V}_\Omega^{(\ell)})^\top  \tilde{\V{\lambda}}_i^{(\ell)} \|_2 = \beta_2 R(\mc{P}^o ({\bf A}_{-i}^{(\ell)}) ), \beta_2 \in [0,1].
\end{equation} 

\textcolor{red}{Note that $\beta_1 = \beta_2$ should hold since both \eqref{eq: 57} and \eqref{eq: 61} correspond to the same problem \eqref{eq: 6}.} This implies
\begin{equation}\label{eq: final1}
\| ({\bf V}_\Omega^{(\ell)})^\top  \tilde{\V{\lambda}}_i^{(\ell)} \|_2 \times r(\mc{P} ({\bf A}_{-i}^{(\ell)}) ) =
\|\tilde{\V{\lambda}}_i^{(\ell)} \|_2 \times r(\mc{P} ({\bf V}_\Omega^{(\ell)} {\bf A}_{-i}^{(\ell)})).
\end{equation}

Since $\tilde{\V{\lambda}}_i^{(\ell)} = (({\bf V}_\Omega^{(\ell)})^\top)^\dagger \bar{\V{\lambda}}_i^{(\ell)}$, we have 
\begin{equation}\label{eq: 62}
({\bf V}_\Omega^{(\ell)})^\top  \tilde{\V{\lambda}}_i^{(\ell)} = \bar{\V{\lambda}}_i^{(\ell)}.
\end{equation}

From \eqref{eq: 8}, \eqref{eq: final1} and \eqref{eq: 62}, we have
\begin{equation} \label{eq: final2}
\left| { ( \bar{ \V {\lambda}}_i^{(\ell)} )^\top }   ({\bf V}_\Omega^{(\ell)})^\dagger  {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)} \right| 
< 
\| \bar{\V{\lambda}}_i^{(\ell)} \|_2 \times r(\mc{P} ({\bf A}_{-i}^{(\ell)}) ),
\end{equation}
which is equivalent to
\begin{equation}
\left| \frac{ ( \bar{ \V {\lambda}}_i^{(\ell)} )^\top }{ {\| \bar{ \V{\lambda}}_i^{(\ell)}\|_2}}   ({\bf V}_\Omega^{(\ell)})^\dagger  {\bf V}_\Omega^{(k)} {\bf a}_j^{(k)} \right| 
< r(\mc{P}({{\bf A}} _{-i}^{(\ell)})).
\end{equation}
Thus we prove our claim. 
%\end{proof}


==> compare_algo.tex <==
Based on Corollary \ref{corollary3}, the probability that SSC-EWZF-LP algorithm succeeds is
\begin{equation} \label{eq: com1}
\begin{split}
& \mathbb{P}(\text{SSC-EWZF-LP})=
\mathbb{P} (
\left|
({\bf Q}_i^{(l)} \V{\lambda}_i^{(l)})^\top {\bf V}_{\Omega_j}^{(k)} {\bf a}_j^{(k)}
\right|
<
1
\\
&: {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)} =\arg \max_{{\bf Q}_i^{(l)} \V{\lambda}_i^{(l)}} \langle {\bf V}_{\Omega_j}^{(l)} {\bf a}_j^{(l)}, {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)}\rangle
\quad \\
& s.t. \quad \| [{\bf V}_{\Omega_1}^{(l)} {\bf a}_1^{(l)},...,{\bf V}_{\Omega_{N_l}}^{(l)} {\bf a}_{N_l}^{(l)}]^\top ({\bf Q}_i^{(l)} \V{\lambda}_i^{(l)})\|_\infty \leq 1 )
\end{split}
\end{equation}

Based on Theorem \ref{theorem}, the probability that SSC-LP algorithm succeeds is
\begin{equation}\label{eq: com2}
\begin{split}
& \mathbb{P}(\text{SSC-LP})=
\mathbb{P} (
\left|
(  {\bf I}_{\Omega_i^{(l)}} {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)})^\top {\bf V}_{\Omega_j}^{(k)} {\bf a}_j^{(k)}
\right|
<
1
\\
&:  {\bf I}_{\Omega_i^{(l)}}  {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)} =\arg \max_{{\bf I}_{\Omega_i^{(l)}} {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)}} 
\langle {\bf V}_{\Omega_j}^{(l)} {\bf a}_j^{(l)},  {\bf I}_{\Omega_i^{(l)}} {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)}\rangle
\quad \\
& s.t. \quad \| [{\bf V}_{\Omega_1}^{(l)} {\bf a}_1^{(l)},...,{\bf V}_{\Omega_{N_l}}^{(l)} {\bf a}_{N_l}^{(l)}]^\top  ({\bf I}_{\Omega_i^{(l)}} {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)}) \|_\infty \leq 1 )
\end{split}
\end{equation}

Thus \eqref{eq: com2} is \eqref{eq: com1} with the constraint that the optimal solution ${\bf Q}_i^{(l)} \V{\lambda}_i^{(l)}$ has to be zero at the location corresponds to ${\bf I}_{\Omega_i^{(l)}}$. The extra constraint will not increase the optimal value $\langle {\bf V}_{\Omega_j}^{(k)} {\bf a}_j^{(k)},  {\bf I}_{\Omega_i^{(l)}} {\bf Q}_i^{(l)} \V{\lambda}_i^{(l)}\rangle$ in \eqref{eq: com2} as compared with \eqref{eq: com1}, indicating the higher probability of success for SSC-LP algorithm as compared with SSC-EWZF-LP algorithm. 

==> implication.tex <==
\textbf{Implications of the condition in Theorem \ref{thm:1}}: 

\begin{enumerate}
\setlength \itemsep{-2pt}
\item We note that the RHS in Equation (\ref{eq:case1}) is the same as the RHS for the full observation case, see \cite{soltanolkotabi2012}. Therefore, the performance degradation in clustering comes from increase in the LHS on an average under missing data.
\item The increase in RHS depends on how badly conditioned $\M{V}_{\Omega}^{(\ell)}$ is. If some of the singular values of $\M{V}_{\Omega}^{(\ell)}$ are very small, it will make the LHS in Equation \ref{eq:case1} large. To further understand this, let us consider a \emph{semi-random} model where in each subspace the data points are generated by choosing $\V{a}_{i}^{(\ell)}$ uniformly randomly on a unit sphere \cite{soltanolkotabi2012}. In this case it is easy to show that $\dfrac{\V{\lambda}_{i}^{(\ell) \top}}{\| \lamil\|_2}$ are also uniformly distributed on the unit sphere \cite{dim_red_sc_ext} and the \emph{expected value} of the LHS becomes $ \dfrac{\|(\vell_{\Omega})^{\dagger} \M{V}_{\Omega}^{(k)}\|_{F}}{d}$. This is essentially the (unnormalized) co-ordinate restricted coherence between subspaces $\ell$ and $k$. 
\item If the subspaces are sufficiently incoherent with the standard basis or satisfy an RIP like property for large enough $|\Omega|$, then the condition number of $\M{V}_{\Omega}^{(\ell)}$ is controlled and one can expect to obtain similar performance as the full observation case.

\item Note that \emph{while in this setting one can ensure perfect clustering, one cannot ensure either perfect subspace identification or completion}. This is because in this case the deterministic necessary conditions for identification and completion \cite{2014arXiv1410.0633P} are not satisfied. This indicates that clustering is an easier problem compared to subspace identification and completion under missing data.
\end{enumerate}


Here we would like to mention that the notion of in-radius is related to the notion of \textbf{permeance} \cite{Lerman2012ArXiv} of data points in a given subspace, quantifying how well the data is distributed inside each subspace. In-radius can be thought of as a worst-case permeance that doesn't scale with the number of data points, while permeance scales with the number of data points and is more of an averaged criteria. Perhaps this is the reason that the primal-dual analysis of SSC under full observation is not able to support the empirical evidence that as the number of points per subspace increases the clustering error goes down dramatically. For subspace clustering such the effect of the number of data points was shown more explicitly in a recent paper \cite{GSC2014}. A connection between these two quantities, namely the in-radius and permeance for subspace clustering under missing data will be undertaken in a future work.\\
We will analyze the more general case next. Analysis of the general case is hard and to gain \emph{insights} we break it up into several results. For this we introduce the following notation. 

==> remain.tex <==


\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c}
      \includegraphics[scale=0.4]{Notation.png}
 \end{tabular}}
  \caption{ Schematic depicting the case when all data is sampled at different locations and the notation for the basis $\M{V}_{\Omega_{i,j}}$ zero-filled and restricted to $\Omega_i$. Here we show for the case when $i =1$.}
  \label{fig:Case2}
\end{figure}

\subsection{Case II}



First we consider the case when $|\oi| = d$, i.e. we want to understand, if a given point is sampled at only $d$ locations, when can SSC-LP correctly assign it to the cluster of points from the same subspace.  Without loss of generality let the point come from the subspace $\ell$.

%Let point $i$ belong to subspace $\ell$. Without loss of generality let $\oil$ correspond to the index set at the first $d$ co-ordinates. Let $ \vell_{\oji}= \mathbf{I}_{\oil \cap \oj^{\ell}} \uell$ where $\mathbf{I}_{\oil \cap \oj^{\ell}}$ denotes the projection onto the (non-zero) co-ordinates in $\oil \cap \oj^{\ell}$. 

%Without loss of generality let $\oil$ correspond to the index set at the first $d$ co-ordinates. 

%\textbf{Notation}: 

%\begin{enumerate}
%\setlength \itemsep{5pt}
%\item Let $\M{V}_{\oi}^{(\ell)} = \M{I}_{\oil} \M{U}^{(\ell)}$. For other data points, $\M{X}_j$ if $\M{X}_j$ belongs to subspace $k \in \{1,2,..,L\}$, $\M{V}_{\Omega_{i,j}^{(k)}} = \M{I}_{\oil} \M{U}^{(k)}$ if $\Omega_{i}^{(\ell)} \subseteq \Omega_{j}^{(k)}$, else $\M{V}_{\Omega_{i,j}^{(k)}} = \M{I}_{\oil \cap \Omega_{j}^{(k)}} \M{U}^{(k)}$, where $\M{I}_{\oil \cap \Omega_{j}^{(k)}}$ is an $|\oil| \times |\oil|$ diagonal matrix with diagonal entries $1$ at locations in   $\M{I}_{\oil \cap \Omega_{j}^{(k)}}$ and $0$ otherwise. This is depicted in Figure, \ref{fig:Case2}.
%\item Let $\M{V}_{\oi}^{(\ell)} = \M{Q}_{i}^{(\ell)} \Sigma_{i}^{(\ell)} \M{R}_{i}^{(\ell) \top}$ and $\M{V}_{\Omega_{i,j}}^{(\ell)} = \M{Q}_{j}^{(\ell)} \Sigma_{j}^{(\ell)} \M{R}_{j}^{(\ell) \top}$ be the SVDs of the truncated basis matrices.
%
%\item Let \begin{align}
%\tilde{\V{a}}_{j}^{(\ell)} &= \M{Q}_{i}^{(\ell) \top} \M{V}_{\oji}^{(\ell)} \aell_{j} \,\,\forall j \\
% & = \M{Q}_{i}^{(\ell) \top} \M{Q}_{j}^{(\ell)} \underset{\hat{\V{a}}_{j}^{(\ell)}}{\underbrace{\Sigma_{j}^{(\ell)} \M{R}_{j}^{(\ell) \top} \aell_{j}}}
%\end{align} and let $\tilde{\M{A}}_{-i}^{(\ell)}$ be the $r \times (N_\ell-1)$ matrix with columns as $\tilde{\V{a}}_{j}^{(\ell)}\,\, , j \neq i$.
%\end{enumerate}

%Under this condition note that $\M{V}_{\oi}^{(\ell)}  \doteq \vell_{\Omega_{i,i}^{(\ell)}}$ is \emph{invertible} if $\M{U}^{(\ell)}$ satisfies the property that any $d \times d$ submatrix is full rank. We will assume this to be true for now.

%We note that this condition is essentially equivalent (under a random sampling) to the condition that the basis $\M{U}^{(\ell)}$ is \emph{not coherent} with the standard basis. 

 
%We consider the following primal problem and its dual.
%\begin{align}
%& P(\M{X}_{\oi}^{(\ell)}, \xell_{-i,\ol})\\
%& = \arg \min \|\V{c}_i^{(\ell)}\|_{1}: \,\, \mathbf{I}_{\oil} \xell_{-i,\ol} \V{c}_{i}^{(\ell)} = \M{X}_{\oi}^{(\ell)}\\
%& D(\M{X}_{\oi}^{(\ell)}, \xell_{-i,\oil})\\
%& = \arg \max \langle \M{X}_{\oi}^{(\ell)}, \V{\nu}_{i}^{(\ell)} \rangle: \,\, \| (\mathbf{I}_{\oil} \M{X}_{-i,\ol}^{(\ell)})^\top \V{\nu}_{i}^{(\ell)}\|_\infty \leq 1
%\end{align}

\textbf{Assumption}: For all possible supports $\Omega_{i}^{(\ell)}$, we assume that  $\M{Q}_{i}^{(\ell)} \in \mb{R}^{d \times d}$ is invertible. This assumption will be satisfied if the columns of $\M{U}^{(\ell)}$ are sufficiently incoherent with the standard basis. Under this assumption, we have the following theorem.
%
%\begin{align}
%P(\tilde{\M{A}}_{-i}^{(\ell)}, \V{a}_{i}^{(\ell)})= \arg \min \|\V{b}_i^\ell\|_{1}: \,\, \tilde{\M{A}}_{-i}^{(\ell)} \V{b}_{i}^{\ell} = \V{a}_{i}^{(\ell)}\\
%D(\tilde{\M{A}}_{-i}^{(\ell)}, \V{a}_{i}^{\ell})= \arg \max \langle \V{a}_{i}^{(\ell)}, \V{z}_{i}^{(\ell)} \rangle: \,\, \| \tilde{\M{A}}_{-i}^{(\ell)\top} \V{z}_{i}^{(\ell)}\|_\infty \leq 1
%\end{align}



 

\begin{theorem}
\label{thm:2}
 Let $|\oil| = d$.  Then SSC-LP correctly assigns it to the data points coming from subspace $\ell$, if for all $k \neq \ell$ and $j$ , the following holds,
\begin{align}
\label{eq:case2}
\left| \frac{\V{\lambda}_{i}^{(\ell) \top}}{\| \lamil\|_2} \M{Q}_{i}^{(\ell)\top} \M{V}_{\Omega_{i,j}}^{(k)} \V{a}_{j}^{(k)} \right| < r_{in}(\mc{P}(\tilde{\M{A}}_{-i}^{(\ell)}))\,\, ,
\end{align} 
where,
\begin{enumerate}
\setlength \itemsep {5pt}
\item $\lamil \in \arg \max_{\V{\lambda}} \langle \hat{\V{a}}_{i}^{(\ell)}, \V{\lambda} \rangle\,\, : \,\, \| \tilde{\M{A}}_{-i}^{(\ell) \top} \V{\lambda}\|_{\infty} \leq 1 $%D(\hat{\V{a}}_{i}^{(\ell)}, \tAell_{-i})$.
\item $\mc{P}(\tAell_{-i}) = \{ \V{v}: \V{v} =  \tAell_{-i} \V{b}: \|\V{b}\|_{1} = 1\}$, and  $r_{in}(\mc{P}(\tilde{\M{A}}_{-i}^{\ell}))$ denotes the in-radius of the centro-symmetric body. 
\end{enumerate}
\end{theorem}

\begin{proof}
The proof follows from slight modifications of the the arguments of the proof of Theorem \ref{thm:1}, which in turn follows from the proof of [Theorem 6 in \cite{dim_red_sc_ext}].%We will now construct a vector $\V{c}_i$ and a dual vector $\V{\nu}_{i}^{(\ell)}$ that satisfies conditions of the Lemma \ref{lem:1} for the problem $P(\M{X}_{\oi}, \M{X}_{-i,\Omega})$. For this we divide $\M{X}_{-i,\Omega}$
%
%Let $\V{c}_{i}^{(\ell)}$ be the solution to $P(\tilde{\M{A}}_{-i}^{(\ell)}, \V{a}_{i}^{\ell})$. Let $$\V{c}_i =[\V{0},...,\V{c}_{i}^{(\ell)},...,\V{0}]^{\top}$$ and $\lamil \in D({\V{a}}_{i}^{(\ell)}, \tAell_{-i})$. Let $\nuil = (\M{V}_{\oi}^{(\ell) \top})^\dagger \lamil$. Then we note that the vectors $\V{c}_i$ and $\nuil$ satisfy the following conditions. 
%
%\begin{enumerate}
%\item For $|\oil| = r$, $P(\tilde{\M{A}}_{-i}^{(\ell)}, \V{a}_{i}^{(\ell)}) = P({\M{X}}_{-i}^{(\ell)}, \M{X}_{i}^{(\ell)}) $ and therefore $\V{c}_{i}$, satisfies $\M{X}_{-i} \V{c}_i = \M{X}_{i}^{(\ell)}$ .  This is because in this case $\M{V}_{\oi}^{(\ell)} (\M{V}_{\oi}^{(\ell)})^{\dagger} = [\M{I}_{r\times r}; \M{0}_{n-r \times n-r}]$. Note that if $|\oil| > r$, then this is no longer true and the resulting analysis is more difficult. However if the conditions of the theorem are satisfied at this sampling rate then it is sufficient for correct clustering.
%\item $(\mathbf{I}_{\oil} \xell_{-i,\ol})^\top \nuil = \mbox{sign}(\V{c}_{i}^{(\ell)}) $. To verify this note that $\V{c}_{i}^{(\ell)}, \lamil$ form a primal-dual pair and, 
%\begin{align}
%(\mathbf{I}_{\oil} \xell_{-i,\ol})^\top \nuil & =  (\mathbf{I}_{\oil} \xell_{-i,\ol})^\top (\M{V}_{\oi}^{(\ell) \top})^\dagger \lamil \\
%& = \tilde{\M{A}}_{-i}^{(\ell) \top} \lamil
%\end{align} 
%\item Clearly we have $\|(\mathbf{I}_{\oil} \xell_{-i,\ol})^\top \nuil\|_{\infty} \leq 1$ 
%\end{enumerate}
%Now, from Lemma \ref{lem:1}, if for all other points $\M{I}_{\oil} \M{V}_{\oj^{(k)}} \V{a}_{j}^{(k)}$, if $| (\M{I}_{\oil} \M{V}_{\oj^{(k)}} \V{a}_{j}^{(k)})^\top \nuil | < 1 $, then there will be no contribution from the columns outside $\M{X}^{(\ell)}$ in expressing the point $\M{I}_{\oil} \M{X}_i$. Substituting $\nuil = (\M{V}_{\oi}^{(\ell) \top})^\dagger \lamil$ in this condition and noting that $ (\M{V}_{\oi}^{(\ell) \top})^\dagger = (\M{V}_{\oi}^{(\ell) \dagger})^\top$ we obtain that, 
%\begin{align}
%\label{eq:cond1}
% \left| \frac{\V{\lambda}_{i}^{(\ell) \top}}{\| \lamil\|_2} (\vell_{\oi})^\dagger \M{V}_{\oj^{(k)} \cap \oil}^{(k)} \V{a}_{j}^{(k)} \right| \leq \frac{1}{\| \lamil \|} 
% \end{align}
%Now note that $\lamil \in \mc{P}(\tAell_{-i}) = \{ \V{z}: \|(\tAell_{-i})^\top \V{z}\|_{\infty} \leq 1\}$. Therefore $\| \lamil \|_2 \leq \mc{R}(\mc{P}(\tAell_{-i}))$ where $\mc{R}(\cdot)$ denotes the circumradius of the cnetro-symmetric body, i.e. the radius of the smallest Euclidean ball in $\mb{R}^{r -1}$ that contains $\mc{P}(\tAell_{-i})$. Noting that the in-radius of a centro-symmetric convex body is inverse of the circumradius of the polar, we obtain that, 
%$$ \| \lamil \|_2 \leq \mc{R}(\mc{P}(\tAell_{-i})) = \frac{1}{r(\mc{P}^{\circ}(\tAell_{-i}))}$$
%Plugging this into Equation \ref{eq:cond1} we obtain the result.
\end{proof}


\textbf{Implications of condition in Theorem \ref{thm:2}}:
\begin{itemize}
\setlength \itemsep{-2pt}


\item The in-radius $r(\mc{P}^{\circ}(\tilde{\M{A}}_{-i}^{(\ell)}))$ now \emph{depends on the sampling pattern within the subspace and it is different for different set of points}. Specifically note that it depends on the \emph{intrinsic subspace coherence} between the sampled points within the same subspace. In general it can be very small if the number of points $\M{X}_{j}^{(\ell)}$ (within the same subspace) that have good amount of overlap with $\M{X}_{i}^{(\ell)}$ is small.

%\item The co-ordinate restricted coherence term, $\M{Q}_{i}^{(\ell)\top} \M{V}_{\Omega_{i,j}}^{(k)}$, depends on the normalized coherence between the subspaces $\ell$ and $k$ when restricted to co-ordinates in $\Omega_{i}^{(\ell)}$. This quantity depends on the condition number of $\vell_{\oi}$, which if bad will make the L.H.S large. If the basis $\M{U}^{(\ell)}$ is highly incoherent with the co-ordinate basis, then this condition number can be controlled. In particular if $\M{U}^{(\ell)}$ satisfies Restricted Isometry Property (RIP) with RIP constants very close to $1$ for sampling factor $d$, then this inverse is well behaved.

%In particular if the following assumption is satisfied,\\
%\textbf{Assumption}: There exists at least $r$ points $\M{X}_{j}^{(\ell)}$ such that $|\Omega_{i}^{(\ell)} \cap \Omega_{j}^{(\ell)}| = r$. \\
%then the in-radius will not shrink too much due to non-overlap. Recall that $\tilde{\V{a}}_{j}^{(\ell)} = (\vell_{\oi})^{-1} \M{V}_{\oji}^{(\ell)} \aell_{j}\,\, , j \neq i$ and if there is not much overlap in the support $(\vell_{\oi})^{-1} \M{V}_{\oji}^{(\ell)}$ can have a bad isometry constant.

\item The subspace coherence also depends on the \emph{relative} sampling pattern of points in other subspaces with respect to the point under consideration. This is reflected in the coherence term $\M{Q}_{i}^{(\ell)\top} \M{V}_{\Omega_{i,j}}^{(k)}$. Unlike Case I, for the semi-random model the distribution of the normalized dual direction is not uniform and we cannot comment on the average case performance. However, a worst-case condition can be obtained here from Equation \ref{eq:case2} which says that if \begin{align} \label{eq:case2a1}
\|\M{Q}_{i}^{(\ell)\top} \M{V}_{\Omega_{i,j}}^{(k)}\|_{2} \leq r_{in}(\mc{P}^{\circ}(\tilde{\M{A}}_{-i}^{(\ell)}))\end{align} then SSC-LP leads to correct clustering. This ofcourse requires that the co-ordinate projected subspaces be sufficiently incoherent as well as \emph{disjoint}.
\end{itemize}

\vspace{-3mm}
\subsection{Case III}

With these \textbf{insights} let us now proceed to handle the more general case when $|\oil| > d$. In order to do that let us first provide a geometric result using Lemma \ref{lem:1} (see Appendix) and then find a useful characterization of the dual certificate.\\


Again let  $\M{V}_{\Omega_i}^{(\ell)} = \M{Q}_{i}^{(\ell)} \Sigma_{i}^{(\ell)} \M{R}_{i}^{(\ell)\top}$ be the SVD of $\M{V}_{\Omega_i}^{(\ell)}$. Let $\M{x}_{\oil,j}$ denote the zero filled $\M{I}_{\Omega_j}\M{X}_j$ restricted to the indices in $\oil$ for all $j \in [N]$. Let $\M{X}_{-i,\oil}$ denote the matrix of these points except point $i$.

 Then SSC-LP solves $ \arg \min \|\V{c}_{i}\|_1: \,\, \M{X}_{i,\oil} = \M{X}_{-i,\oil} \V{c}_{i} $. Let $\V{c}_{i}^{(\ell)}$ and $\V{\nu}_{i}^{(\ell)}$ be solutions to,
$$ \arg \min \|\V{b}\|_1: \,\, \M{X}_{i,\oil}^{(\ell)} = \M{X}_{-i,\oil}^{(\ell)} \V{b}$$ 
$$ \arg \max \langle \M{X}_{i,\oil}^{(\ell)}, \V{\nu} \rangle: \,\, \| \M{X}_{-i,\oil}^{(\ell)\top} \V{\nu}\|_\infty \leq 1 $$ 

\noindent Assuming that \emph{strong duality} holds, the vectors $$\V{c} = [ \V{0},\cdots, \V{0}, \V{c}_{i}^{(\ell)},\cdots, \V{0}]^\top$$ and $\V{\nu}_{i}^{(\ell)}$ satisfy the conditions of Lemma \ref{lem:1} (See Appendix), hence guaranteeing correct subspace recovery if for all $k \neq \ell, j$, the following condition is satisfied. 
\begin{align} | \V{\nu}_{i}^{(\ell)\top} \M{X}_{\oil,j}^{(k)}| < 1 \end{align}
%Note that, $\M{X}_{\oil,j}^{(k)}$ is the zero filled vector from subspace $k$ restricted to the support $\oil$. 

As such this condition does not provide any further intuition or insights. In order to arrive at results that are similar in flavor to Theorems \ref{thm:1} and \ref{thm:2}, let us further analyze this condition. We have the following \textbf{Assumption}: The matrix $\M{Q}_{i}^{(\ell)}$ has full column rank. This assumption is satisfied if columns of $\M{U}^{(\ell)}$ are sufficiently incoherent with respect to the co-ordinate basis.

Let $\M{Q}_{i}^{(\ell)} \M{Q}_{i}^{(\ell)\top}$ denote the projection matrix that projects a vector onto the subspace spanned by columns of $\qil \qilt$ and $(\M{I} - \qil \qilt)$ denote the null space of $\qilt$. Note that, $$\nuil =  \qil \qilt \nuil + (\M{I} - \qil \qilt)\nuil .$$ 
Then the condition for correct clustering becomes,
\begin{align} | ( \qil \qilt \nuil + (\M{I} - \qil \qilt)\nuil)^{\top} \M{X}_{\oil,j}^{(k)}| \leq 1 \end{align}
By triangle inequality if for some $0\leq \alpha \leq 1$, 
\begin{align}
\label{eq:case3a1} | (\nuil)^{\top} \M{Q}\M{Q}^{\top} \M{X}_{\oil,j}^{(k)}| < \alpha \end{align} 
and
\begin{align}
\label{eq:case3b1}
| (\nuil)^{\top} ( \M{I} - \M{Q}\M{Q}^{\top}) \M{X}_{\oil,j}^{(k)}| \leq (1-\alpha)
\end{align}
then the point $\M{X}_{i}^{(\ell)}$ is correctly clustered. Based on this we have the following theorem.

\begin{theorem}
\label{thm:3}
If for any point $\M{x}_i$ belonging to subspace $\ell$, the following conditions are satisfied,
\begin{align}
\label{eq:case3a}
\|\M{Q}_{i}^{(\ell)\top} \M{V}_{\Omega_{i,j}}^{(k)}\|_{2} < \alpha r_{in}\left(\mc{P}(\M{X}_{-i,\oil}^{(\ell)\top})\right)
\end{align}
\begin{align}
\|(\M{I} - \qil \qilt) \M{V}_{\Omega_{i,j}}^{(k)}\|_{2} \leq (1- \alpha) r_{in}\left(\mc{P}(\M{X}_{-i,\oil}^{(\ell)})\right)
\end{align}
for some $0 \leq \alpha \leq 1$, then SSC-LP succeeds. Here $\mc{P}(\M{X}_{-i,\oil}^{(\ell)}) = \{ \V{v}: \V{v} =  \M{X}_{-i,\oil}^{(\ell)} \V{b}: \|\V{b}\|_{1} = 1\}$, and  $r_{in}(\mc{P}(\M{X}_{-i,\oil}^{(\ell)}))$ denotes the in-radius of the centro-symmetric body
\end{theorem}
We note the following points. 
\begin{enumerate}
\item Compared to Theorems \ref{thm:1} and \ref{thm:2}, the conditions stated in Theorem \ref{thm:3} are worst-case and slightly weaker in the sense that they require the co-ordinate projected  subspaces to be disjoint.

\item Also note that for the most general case it is required that \emph{co-ordinate restricted subspace coherence} be small BUT ALSO that the \emph{projection error of the other set of points} onto the co-ordinate restricted subspace for the point under consideration be small. When $|\oil|$ is large, Equation \ref{eq:case3a} is more likely to be satisfied compared to Equation \ref{eq:case2a1}.

\item In the most general case, while more observations (per vector) is required, in this case under correct clustering if the sampling patterns and the number of data points satisfy the necessary and sufficient conditions in \cite{2014arXiv1410.0633P,2015arXiv150302596P} then it is possible to also correctly identify the subspaces and also ensure completion.
\end{enumerate}


%We now make the following claims. 
%
%\noindent \textbf{Claim 1}:  The vector $ \M{Q}\M{Q}^\top \nuil$ is one of the solutions to 
%\begin{align}
%\label{eq:11} \arg \max \langle \M{X}_{i,\Omega_o}^{(\ell)}, \V{\nu}' \rangle: \,\, \| \M{X}_{-i,\Omega_o}^{(\ell)\top} \M{Q}\M{Q}^\top \V{\nu}'\|_\infty \leq \eta\end{align} for some $\eta \geq 1$.\\
%
%\noindent \textbf{Claim 2}:  Any solution $\V{\nu}^*$ to Equation \ref{eq:11} can be written as $\V{\nu}^* = \qil \V{\lambda}^*$ where $\V{\lambda}^*$ is one of the solutions to  
%\begin{align}
%\label{eq:12} \arg \max \langle \hat{\V{a}}_{i}^{(\ell)}, \V{\lambda} \rangle: \,\, \| (\qilt \M{X}_{-i,\Omega_o}^{(\ell)})^\top \V{\lambda}\|_\infty \leq \eta
%\end{align}
%Recall from Equation \ref{eq:hata1} that Equation \ref{eq:12} is by definition equivalent to,
%\begin{align}
%\label{eq:12a} \arg \max \langle \hat{\V{a}}_{i}^{(\ell)}, \V{\lambda} \rangle: \,\, \|  \tilde{\M{A}}_{-i}^{(\ell)\top} \V{\lambda}\|_\infty \leq \eta
%\end{align}
%Combining these results we have the following main Theorem.
%\begin{theorem}
%\label{thm:3}
%SSC-EWZF correctly clusters the point $\M{X}_i$ under missing data, i.e. assigns it to the data points coming from subspace $\ell$, if for all $k \neq \ell$ and $j$, the following holds,
%\begin{align}
%\label{eq:case3a}
%\left| \frac{\V{\lambda}_{i}^{(\ell) \top}}{\| \lamil\|_2} \M{Q}_{i}^{(\ell)\top} \M{V}_{\Omega_{i,j}}^{(k)} \V{a}_{j}^{(k)} \right| < \frac{1}{2 \eta} r_{in}(\mc{P}^{\circ}(\tilde{\M{A}}_{-i}^{(\ell)}))\,\, ,
%\end{align} 
%\begin{align}
%\label{eq:case3b}
%\|(\M{I} - \qil \qilt) \M{X}_{\oil,j}^{(k)}\|_{2} \leq \frac{1}{2} r_{in}(\mc{P}(\M{X}_{-i,\oil}^{(\ell)}))
%\end{align}
%where,
%\begin{enumerate}
%\setlength \itemsep {5pt}
%\item $\lamil \in \arg \max_{\V{\lambda}} \langle \hat{\V{a}}_{i}^{(\ell)}, \V{\lambda} \rangle\,\, : \,\, \| \tilde{\M{A}}_{-i}^{(\ell) \top} \V{\lambda}\|_{\infty} \leq \eta $%D(\hat{\V{a}}_{i}^{(\ell)}, \tAell_{-i})$.
%
%\item $\mc{P}^{\circ}(\tAell_{-i}) = \{ \V{v}: \V{v} =  \tAell_{-i} \V{b}: \|\V{b}\|_{1} = 1\}$, and  $r_{in}(\mc{P}^{\circ}(\tilde{\M{A}}_{-i}^{\ell}))$ denotes the in-radius of the centro-symmetric body. 
%
%\item $\mc{P}(\M{X}_{-i,\oil}^{(\ell)}) = \{ \V{v}: \V{v} =  \M{X}_{-i,\oil}^{(\ell)} \V{b}: \|\V{b}\|_{1} = 1\}$, and  $r_{in}(\mc{P}(\M{X}_{-i,\oil}^{(\ell)}))$ denotes the in-radius of the centro-symmetric body. 
%
%\end{enumerate}
%
%\end{theorem} 


%In order to lower bound the in-radius when compared to Case I, we make the following assumption.
%
%\textbf{Assumption}: For each $\M{X}_{\oi}^{(\ell)}$ there exists at-least $r$ data points $\M{X}_{\oj}^{(\ell)}$ such that $|\oil \cap \oj^{(\ell)} | \geq r$.
%
%While this assumption is not necessary, it is to ensure that the in-radius, which will be dominated by how the points are sampled relative to each other, will remain almost the same as when fully sampled case. If this condition is not satisfied, then within the same subspace, some of the points may not contribute well for a minimal linear contribution to represent the point under consideration. Further this assumption may be relaxed if after sampling the points are re-normalized. This is borne out by the following analysis. Note that,   
%If cardinality of the set $\{ \M{X}_{j}^{(\ell)}: |\oil \cap \Omega_{j}^{(\ell)}| \geq r \}$ is smaller than $r$ then the matrix $\tilde{\M{A}}_{-i}^{(\ell)}$ will be rank deficient, in that the rank of the matrix will be $< r$ and one cannot ensure that $r(\mc{P}^{\circ}(\tilde{\M{A}}_{-i}^{\ell})) > 0$ in this case. It is important to note here that we are talking about the maximum radius of an $r$-ball that can fit inside the polytope. If we were to ask the maximum in-radius of an $(r-1)$-ball the in-radius will be larger \cite{Gritzmann92}. This justifies Assumption 2. Again note that in \cite{icml2015_wange15} this assumption is already satisfied owing to the fact that $\Omega$ is fixed for each data point. 

%\textcolor{red}{Wenqi: If we project all the data onto the same $\Omega$ and if $|\Omega| \geq r +1$, then can one identify the subspace from this sampling pattern? Answer: We cannot identify the subspace as the sampling patterns don't satisfy the necessary conditions in \cite{Pimentel}}. 

%Moreover in the noiseless sampling setting of \cite{icml2015_wange15}, the analysis using the linear program is trivial since $\tilde{\V{a}}_{i}^{(\ell)} = \V{a}_{i}^{(\ell)}$ and the in-radius will not change. Further, if  $ \V{a}_{i}^{(\ell)}$ are uniformly distributed on the unit sphere, then $\dfrac{\V{\lambda}}{\|\V{\lambda}\|}$ will also be uniformly distributed on the unit sphere and thereby replicating the analysis in \cite{1,2}, one can bound the subspace-incoherence term in a simple manner. 
%\begin{align}
%\tilde{\V{a}}_{j}^{(\ell)} = ( \uellt \mathbf{I}_{\oil} \uell)^{-1} \M{U}^{(\ell) \top} \mathbf{I}_{\oil \cap \oj^{(\ell)}} \uell \V{a}_{j}^{(\ell)}
%\end{align}
%If $|\oil| \geq r$ and if $|\oil \cap \oj^{(\ell)}| \geq r$, then the matrix $(\M{U}^{(\ell)\top} \mathbf{I}_{\oil} \uell)^{-1} \M{U}^{(\ell) \top} \mathbf{I}_{\oil \cap \oj^\ell} \uell$ is invertible and 
%\begin{align}
%\|\tilde{\V{a}}_j^{(\ell)}\|_{2} & \geq \sigma_{\min}\left((\M{U}^{(\ell)\top} \mathbf{I}_{\oil} \uell)^{-1}\right) \sigma_{\min} \left(\M{U}^{(\ell) \top} \mathbf{I}_{\oil \cap \oj^\ell} \uell \right) \|\V{a}_{j}^{(\ell)}\|_2 \\
%& = \frac{\sigma_{\min} \left(\uellt \mathbf{I}_{\oil \cap \oj^\ell} \uell \right)}{\sigma_{\max}(\M{U}^{(\ell)\top} \mathbf{I}_{\oil} \uell)} \|\V{a}_{j}^{(\ell)}\|_2  \geq  \frac{\sigma_{\min} \left(\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell \right)}{\sigma_{\max}(\M{U}^{(\ell)\top} \mathbf{I}_{\oil} \uell)} \|\V{a}_{j}^{(\ell)}\|_2
%\end{align}   
%Let $\uell, \ell = 1,2,...,L$ satisfy the property that for all $\Omega: |\Omega| \geq r$, the condition number of $\M{U}^{(\ell)\top} \mathbf{I}_{\Omega} \uell$ is $\geq \tau_0 > 0$, then from the above Equations it is clear that, 
%$$ r(\mc{P}^{\circ}(\tilde{\M{A}}_{-i}^{(\ell)})) \geq \tau_0 r(\mc{P}^{\circ}({\M{A}}_{-i}^{(\ell)}))$$ 

%\textcolor{blue}{We will now show that $\tau_0$ is positive with high probability under sufficiently high sampling rate with uniform sampling. Clearly, $\sigma_{\max}(\M{U}^{(\ell)\top} \mathbf{I}_{\oil} \uell) \leq 1$. Let $\mu$ denote the incoherence of the subspace defined as $\mu = \max_{j} \frac{n}{r} \| \M{U}^{(\ell)\top} \V{e}_j\|_{2}^{2}$, where $\V{e}_j$ denotes the $j$-th unit vector in $\mb{R}^{n}$. From [\cite{Balzano_ISIT2010}, Lemma 3] as long as $|\Omega_i| \geq \frac{8}{3}r \mu \log(2r/\delta)$ it follows that, with probability $> 1 - \delta$, $\sigma_{\min} \left(\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell \right) \geq \frac{|\Omega_i|(1-\gamma)}{n}$ for some $\gamma <1$. Therefore we can fix $\tau_0 = \frac{3 r \mu \log (2r/\delta)(1-\gamma)}{n}$ for some small enough $\gamma$ and $\delta$.}


%\textcolor{red}{We need to do some kind of expected analysis, with expectation over the random sampling}.
%\subsection{Results for the semi-random model}
%In order to derive meaningful results we will adopt a semi-random model  and use concentration of measure results to lower bound the L.H.S. which is the subspace coherence term under random sampling $\left| \frac{\V{\lambda}_i^\ell}{\| \V{\lambda}_i^\ell\|_2} (\M{V}_{\oi}^{\ell})^\dagger \M{V}_{\oj}^{k} \V{a}_{j}^{k} \right| $. 
%
%\textbf{Semi-random model}: Under the semi-random model, the points $\V{a}_{i}^{(\ell)}$ are drawn uniformly from the unit sphere. 
%
%Now note that, 
%\begin{align}
% (\M{V}_{\oi}^{\ell})^\dagger \M{V}_{\oj}^{k}   = (\M{V}_{\oi}^{(\ell)})^\dagger \M{V}_{\oj^{(k)} \cap \oil}^{(k)}  = (\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell)^{-1} \M{U}^{(\ell) \top} \mathbf{I}_{\oil \cap \oj^{(k)}} \M{U}^{(k)} 
%										      %& = (\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell)^{-1} \left(\M{U}^{(\ell) \top} \M{U}^{(k)} + \M{U}^{(\ell) \top} (\M{I} - \mathbf{I}_{\oil \cap \oj^{(k)}}) \M{U}^{k}\right)
%\end{align}
%In the worst case we have $\oil \cap \oj^{(k)} = \oil$ and therefore we need to find a tight upper bound to 
%\begin{align}
%\left| \frac{\V{\lambda}_{i}^{(\ell)\top}}{\| \V{\lambda}_{i}^{(\ell)}\|_2} (\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell)^{-1} \M{U}^{(\ell) \top} \mathbf{I}_{\oil} \M{U}^{(k)} \V{a}_{j}^{k} \right| \end{align}
%Note that since $\V{a}_{i}^{(\ell)}$ are random, the points $\tilde{\V{a}}_{i}^{(\ell)}$ are also random. But unlike the full observation case these points are uniformly distributed on the unit sphere and consequently $\frac{\V{\lambda}_{i}^{(\ell)}}{\|\V{\lambda}_{i}^{(\ell)}\|_{2}}$ are also not uniformly distributed on the unit sphere. Therefore, we can only derive a worst case condition here. We have the following Lemma taken from \cite{XX}.


%Therefore we have, 
%\begin{align}
%\left| \V{x}^\top (\M{V}_{\oi}^{(\ell)})^\dagger \M{V}_{\oj}^{(k)} \V{y} \right| &= \left| \V{x}^\top (\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell)^{-1} \left(\M{U}^{(\ell) \top} \M{U}^{(k)} + \M{U}^{(\ell) \top} (\M{I} - \mathbf{I}_{\oil \cap \oj^{(k)}}) \M{U}^{(k)}\right) \V{y} \right| \\
%& \leq \left| \V{x}^\top (\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell)^{-1} \M{U}^{(\ell) \top} \M{U}^{(k)} \V{y} \right| + \left| \V{x}^\top \M{U}^{(\ell) \top} (\M{I} - \mathbf{I}_{\oil \cap \oj^{(k)}}) \M{U}^{(k)}\V{y} \right| 
%\end{align}
%In the worst case we have 



%We will further simplify the analysis using Assumption 2. In this case we modify the algorithm to collect only those vectors that have an overlap of $\geq r+1$. Then for $|\Omega_{i}^{(\ell)}| = r+1$, for that algorithm, it can be shown that $\tilde{\V{a}}_{i}^{(\ell)} = {\V{a}_{i}^{(\ell)}}$ and therefore  $\lambda_{i}^{(\ell)}$ are uniformly distributed. 
%
%\begin{align}
%\left| \V{x}^\top (\M{V}_{\oi}^{(\ell)})^\dagger \M{V}_{\oj}^{(k)} \V{y} \right| &= \left| \V{x}^\top (\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell)^{-1} \left(\M{U}^{(\ell) \top} \M{U}^{(k)} + \M{U}^{(\ell) \top} (\M{I} - \mathbf{I}_{\oil \cap \oj^{(k)}}) \M{U}^{(k)}\right) \V{y} \right| \\
%& \leq \left| \V{x}^\top (\M{U}^{(\ell) \top} \mathbf{I}_{\oil} \uell)^{-1} \M{U}^{(\ell) \top} \M{U}^{(k)} \V{y} \right| + \left| \V{x}^\top \M{U}^{(\ell) \top} (\M{I} - \mathbf{I}_{\oil \cap \oj^{(k)}}) \M{U}^{(k)}\V{y} \right| 
%\end{align}



%Therefore, we obtain the following theorem.

%\textcolor{red}{Wenqi, start putting in selected results in this section.}

%
%\section{Some implications} 
%
%\begin{enumerate}
%\item The problem of identifying the union of subspace model under missing data implies identification of each of the subspaces from correct clustering. From a recent result \cite{Pimental} it follows that such an identification is not possible unless \textcolor{red}{unless $|\oil| \geq r+1$ and the number of points per subspace, $N_\ell$ satisfy $\sum_{i=1}^{N_\ell}(|\oil|) \geq r(n-r)$ in addition to a condition that the - Wenqi can we summarize the condition?}. This assumption and necessity is in contrast to the full data case when in an ideal case it is sufficient to have $d_\ell$ (linearly independent) points from subspace $\mb{S}^{(\ell)}$. 
%
%\item The problem of clustering and completion is a fundamentally different problem than clustering under missing data. For both clustering and completion, it is required that the number of data points per subsRapace is at-least $d_{\ell} (d-d_\ell)$.
%\end{enumerate}

\begin{figure}[htbp]
\centering
\vspace{-25mm}
\includegraphics[ width = .35\textwidth]{ClusteringError_50_3_3_150_100_Cas1_V2.pdf} 
 \vspace{-23mm}
\caption{Clustering error in the first case (points sampled at same $pn$ co-ordinates)  for varying $p$.}
\end{figure}


\begin{figure*}[t!]
	\centering
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
	\includegraphics[trim=.45in 1.5in .8in 2.8in, clip, width = \textwidth]{ClusteringError_50_3_3_150_100.pdf}\vspace{-.3in}
		\caption{Clustering Error}
	\end{subfigure}%
	~ 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
	\includegraphics[trim=.6in 1.5in .8in 2.8in, clip, width = \textwidth]{CompletionError_50_3_3_150_100.pdf}\vspace{-.3in}
		\caption{Completion Error}
	\end{subfigure}
		~ 
		\begin{subfigure}[b]{0.32\textwidth}
			\centering
			      \includegraphics[trim=.5in 1.5in .8in 2.8in, clip, width = \textwidth]{SubspaceError_50_3_3_150_100.pdf}\vspace{-.3in}
			      \caption{Subspace Error}
		\end{subfigure}
	\caption{Different error metrics  for the case of random sampling.} \label{fig:tensor}\vspace{-.1in}
\end{figure*}

\vspace{-10mm}


==> remark.tex <==
{\remark \label{remark_fact} Equation \label{remark} \eqref{eq:theorem_eq} in Theorem \ref{theorem} is equivalent to
\begin{equation}\label{eq: remark_eq}
\left|  \langle {\bf w}_i^{(\ell)}  , \tilde{\bf{a}}_j^{(k)} \rangle \right| < r(\mc{P}(\tilde{{\bf A}}_{-i}^{(\ell)}))
\end{equation}
where ${\V \lambda}_i^{(\ell)} \in \arg \max_{\V \lambda} \langle \tilde{{\bf a}}_i^{(\ell)}, {\V \lambda} \rangle \quad s.t. \quad \|(\tilde{{\bf A}}_{-i}^{(\ell)})^\top {\V \lambda}\|_\infty \leq 1$, ${\bf w}_i^{(\ell)} = \frac{{\V \lambda}_i^{(\ell)}}{\|{\V \lambda}_i^{(\ell)}\|_2} $
\endremark
}
